A Deep Learning Based Cost Model for Automatic Code Optimization

Enabling compilers to automatically optimize code has been a longstanding goal for the compiler community. Efficiently solving this problem requires using precise cost models. These models predict whether applying a sequence of code transformations reduces the execution time of the program. Building an analytical cost model to do so is hard in modern x86 architectures due to the complexity of the microarchitecture. In this paper, we present a novel deep learning based cost model for automatic code optimization. This model was integrated in a search method and implemented in the Tiramisu compiler to select the best code transformations. The input of the proposed model is a set of simple features representing the unoptimized code and a sequence of code transformations. The model predicts the speedup expected when the code transformations are applied. Unlike previous models, the proposed one works on full programs and does not rely on any heavy feature engineering. The proposed model has only 16% of mean absolute percentage error in predicting speedups on full programs. The proposed model enables Tiramisu to automatically find code transformations that match or are better than state-of-the-art compilers without requiring the same level of heavy feature engineering required by those compilers.

==> sections/broad_impact.tex <==
\section{Broader Impact}
Designing fully-automatic high-performance compilers has a strong impact on many areas. In the area of deep learning, for example, today’s deep learning models are $300000\times$ more computationally intensive than those developed in 2012. An efficient implementation of a model requires writing complex code transformations. Applying all of these transformations requires expertise, is time-consuming, error-prone, and makes the model non-portable. The level of complexity becomes much higher with differentiable programming, where users can train arbitrary differentiable programs instead of being restricted
to a limited set of DNN operators. The same applies to other areas such as HPC (High Performance Computing).

This work has the following potential positive impact in the society: first, it will enable more productivity in writing high-performance software. Second, it will open the door to non computer scientists to write a simple high level code and rely on compilers to automatically optimize it. Third, it will reduce errors and bugs in software.

Failure of fully automatic code optimization does not have dangerous results. First, we guarantee that all the transformations applied are correct (preserve the semantics of programs). If automatic optimization fails, the resulting program will be slower than expected. In that case, the user can disable fully automatic code optimization.

\clearpage

